Shared Adversarial Unlearning: Backdoor Mitigation by Unlearning Shared Adversarial Examples

Backdoor attacks are serious security threats to machine learning models where an adversary can inject poisoned samples into the training set, causing a backdoored model which predicts poisoned samples with particular triggers to particular target classes, while behaving normally on benign samples. In this paper, we explore the task of purifying a backdoored model using a small clean dataset. By establishing the connection between backdoor risk and adversarial risk, we derive a novel upper bound for backdoor risk, which mainly captures the risk on the shared adversarial examples (SAEs) between the backdoored model and the purified model. This upper bound further suggests a novel bi-level optimization problem for mitigating backdoor using adversarial training techniques. To solve it, we propose Shared Adversarial Unlearning (SAU). Specifically, SAU first generates SAEs, and then, unlearns the generated SAEs such that they are either correctly classified by the purified model and/or differently classified by the two models, such that the backdoor effect in the backdoored model will be mitigated in the purified model. Experiments on various benchmark datasets and network architectures show that our proposed method achieves state-of-the-art performance for backdoor defense.

==> backups/method_20230511.tex <==
In Section~\ref{sec::pre}, we first introduce notations, threat model, and defense goal to formulate the problem. By investigating the relationship between adversarial risk and backdoor risk, a new bound of backdoor risk is provided in Section~\ref{sec::risk}, from which a bi-level objective is proposed in Section \ref{sec::loss}.


\subsection{Preliminary}
\label{sec::pre}

\paragraph{Notations.} 
 Let lowercase symbols and lowercase boldface symbols denote scalars and vectors, respectively. Let uppercase calligraphic symbols denote sets/spaces. We consider a $K$-class ($K\geq 2$) classification problem that aims to predict the label $y\in \gY$ of a given sample $\vx \in \gX$, where $\gY=[1, \cdots, K]$ is the set of labels and $\gX$ is the space of samples. Let $h_{\vtheta}:\gX\to \gY$ be a DNN classifier with model parameter $\vtheta$. We use $\gD$ to denote the set of data $(\vx,y)$. For simplicity, we use $\vx\in \gD$ as a abbreviation for $(\vx,y)\in \gD$. Then, for a sample $\vx\in \gD$,  its predicted label is
\begin{equation}
    \htt(\vx) = \argmax_{k=1,\cdots, K} \vp_k(\vx,\vtheta), 
\end{equation}
where $\vp_k(\vx,\vtheta)$ is the (softmax) probability of $\vx$ belonging to class $k$. 

\paragraph{Threat model.}
Let $\gV$ be the set of triggers and define $g:\gX\times \gV \to \gX$ as the generating function for poisoned samples. Then, given a trigger $\Delta \in \gV$ and a sample $\vx\in \gX$, one can generate a poisoned sample $g(\vx,\Delta)$. For simplicity, we only consider all to one case, i.e., there is only one trigger $\Delta$ and one target label $\hat{y}$. The all2all case and multi-trigger case are left in the appendix. We assume that the attacker has access to manipulate the dataset and/or control the training process such that the trained model classifies the samples with pre-defined trigger $\Delta$ to the target labels $\hat{y}$ while classifying clean samples normally.  In addition, we define the poisoning ratio as the proportion of poisoned samples in the training dataset. 

\paragraph{Defense goal.}
We consider that the defender is given a backdoored model with parameter $\theta_{bd}$ and a small set of \textit{clean} data $\Db=\{(\vx_i,y_i)\}_{i=1}^N$. Since we are mainly interested in samples whose labels are not the target label, we further define the set of non-target samples as $\Dn = \{(\vx,y) |(\vx,y) \in \Db, y\neq \hat{y}\}$. Note that the size of $\Db$ is small and the defender cannot train a new model from scratch using $\Db$. The defender's goal is to purify the model so that the clean performance is maintained and the backdoor effect is removed or mitigated. We assume that the defender has neither access to the trigger $\Delta$ nor the target label $\hat{y}$.

\paragraph{Problem formulation.}
Using the $0$-$1$ loss \cite{ wang2020improving, zhang2019theoretically}, the classification risk $\gR_{cl}$ and the backdoor risk $\gR_{bd}$ with respect to classifier $\htt$ on $\Db$ can be defined as:
\begin{align}
    \label{eq::risk}
    \gR_{cl}(\htt) = \frac{1}{N}\sum_{i=1}^N \ind(\htt(\vx_i)\neq y_i), \quad
    \gR_{bd}(\htt) = \frac{\sum_{i=1}^N \ind(\htt(g(\vx_i,\Delta))=\hat{y}, \vx_i\in \Dn)}{|\Dn|}%{\sum_{j=1}^N \ind(y_j\neq \hat{y})},
\end{align}
where $\ind$ is the indicator function and $|\cdot|$ means the cardinality of a set.

In (\ref{eq::risk}), the classification risk concerns whether a clean sample is  correctly classified, while the backdoor risk measures the risk of classifying a poisoned sample to target class if its ground truth label is not $\hat{y}$. 

% Since the backdoor risk only focuses on breaking the relationship between trigger $\Delta$ and target label $\hat{y}$, merely minimizing $\gR_{bd}(\htt)$ may lead to an unacceptable increase of $\gR_{cl}(\htt)$. 
In this paper, we consider the following problem for purifying a backdoored model:
\begin{equation}
    \label{eq::trade}
    \min_{\vtheta} \gR_{cl}(\htt) + \lambda \gR_{bd}(\htt),
\end{equation}
where $\lambda$ is a hyper-parameter to control the tradeoff between classification risk and backdoor risk.

\subsection{Backdoor risk and adversarial risk}
\label{sec::risk}
Since neither the trigger $\Delta$ nor target label $\hat{y}$ is accessible to the defender, directly minimizing (\ref{eq::trade}) is impractical. A natural way is to replace the poisoned samples with adversarial examples (AEs) \cite{chai2022oneshot,zeng2022adversarial}. Therefore, we delve deeper into the relationship between adversarial risk and backdoor risk in this section.

Let $\gS$ be a set of perturbations. Given a sample $\vx$ and an adversarial perturbation $\veps$, an adversarial example $\tilde{\vx}(\veps)$ can be generated by $\tilde{\vx}(\veps) = \vx+\veps$. We define the set of adversarial example-label pair for $\htt$ generated by perturbation $\veps$ and dataset $\Db$ by
$\gA(\veps,\vtheta)=\{(\tilde{\vx}(\veps),y)|\htt(\tilde{\vx}(\veps))\neq y, (\vx,y)\in \Db\}$ and abbreviate $(\tilde{\vx}(\veps),y) \in \gA(\veps,\vtheta)$ by $\tilde{\vx}(\veps) \in \gA(\veps,\vtheta)$. Then, the adversarial risk for $\htt$ on $\Dn$ can be defined as
\begin{equation}
    \label{eq::ae_risk}
    \gR_{adv}(\htt) = \frac{\sum_{i=1}^N \max_{\veps_i \in \gS}\ind(\tilde{\vx}_i(\veps_i) \in \gA(\veps_i,\vtheta), \vx_i\in\Dn)}{|\Dn|}.%{\sum_{j=1}^N \ind(y_j\neq \hat{y})}.
\end{equation}

To bridge the adversarial examples and poison samples, we provide the following assumption:
\begin{assumption}  
\label{assm:S}
Assume that $g(\vx,\Delta) - \vx \in \gS$ for  $\forall \vx \in \Db$.
\end{assumption}

Assumption \ref{assm:S} ensures that there exists $\veps \in \gS$ such that $\vx+\veps = g(\vx,\Delta)$. As poisoned samples are required to be imperceptible to humans, Assumption \ref{assm:S} is quite mild. For example, an $L_p$ ball with radius $\rho$, i.e., $\gS=\{\veps |\|\veps\|_p\leq \rho \}$, is sufficient to satisfy Assumption \ref{assm:S} with proper $p$ and $\rho$.

\begin{figure}[t]
    \centering
    \includegraphics[width = 0.9\linewidth]{images/decision_boundary_type.pdf}
    \caption{Illustration of the Shared Adversarial Example for the current classifier $\htt$ and the backdoored classifier $\hbd$. Assume that $ \htt(g(x,\Delta))=\hbd(g(x,\Delta))=\hat{y}$ and the target label is~$3$. The adversarial examples for $\hbd$ and $\htt$ are marked with blue and green, respectively. The shared adversarial examples which mislead $\hbd$ and $\htt$ to the same class are marked with red and the poisoned sample is denoted by the pentagram.}
    \label{fig::cup}
\end{figure}



To generate the adversarial example for sample $\vx$, a typical way is to compute $\veps$ that maximizes the misclassification risk of $\tilde{\vx}(\veps)$ measured by some loss functions \cite{madry2018towards, wang2020improving}. However, such a process misses some intrinsic connections between adversarial examples and poisoned samples. Given a backdoored model $\hbd$, the adversarial examples to $\htt$ generated from $\vx$ can be categorized into 4 types as summarized in Table~\ref{tab:AE}:

\begin{table}[h]
  \caption{Category of Adversarial Examples from $\vx$ }
  \label{tab:AE}
  \centering
  \begin{tabular}{lll}
    \toprule
    \cmidrule(r){1-3}
    Type     & Description     & Definition \\
    \midrule
    \RNum{1}       & Mislead $\hbd$ only   & $\hbd(\tilde{\vx}(\veps))\neq y, \htt(\tilde{\vx}(\veps)) = y$     \\
    \RNum{2}       & Mislead $\htt$ only & $\hbd(\tilde{\vx}(\veps)) = y, \htt(\tilde{\vx}(\veps))\neq y$     \\
    \RNum{3}      & Mislead $\hbd$ and $\htt$ to the same class       & $\hbd(\tilde{\vx}(\veps)) = \htt(\tilde{\vx}(\veps))\neq y$ \\
    \RNum{4}       & Mislead $\hbd$ and $\htt$ to different classes  & Others     \\
    \bottomrule
  \end{tabular}
\end{table}

% 1) AEs that merely mislead $\hbd$; %, i.e., $\Sbd(\vx) = \{\veps\in \gS|\hbd(\tilde{\vx}(\veps))\neq y, \htt(\tilde{\vx}(\veps))= y\}$; 
% 2) AEs that merely mislead $\htt$; %, i.e., $\Stt(\vx) = \{\veps\in \gS|\hbd(\tilde{\vx}(\veps)) = y, \htt(\tilde{\vx}(\veps))\neq y\}$;
% 3) common AEs that mislead $\htt$ and $\hbd$ to different classes; %, i.e., $\Scom(\vx) = \{\veps\in \gS|\hbd(\tilde{\vx}(\veps)) \neq y, \htt(\tilde{\vx}(\veps))\neq y, \hbd(\tilde{\vx}(\veps)) \neq \htt(\tilde{\vx}(\veps))\}$;
% 4) shared AEs that mislead $\htt$ and $\hbd$ to the same class. %, i.e., $\Ssha(\vx) = \{\veps\in \gS|\hbd(\tilde{\vx}(\veps))= \htt(\tilde{\vx}(\veps))\neq y\}$.

Let $\Ds = \{(\vx,y)|\hbd(g(\vx, \Delta))=\hat{y}, \vx\in \Dn\}$ be the subset of samples in $\Dn$ on which planting a trigger can successfully activate the backdoor in $\hbd$ and denote its complementary by $\Df = \Dn\setminus\Ds$. Then, the following proposition reveals a deeper connection between adversarial example and poisoned samples as illustrated in Figure~\ref{fig::cup}:

\begin{proposition} 
\label{ass:share}
For $\forall (\vx,y) \in \Ds$, the poisoned sample $g(\vx, \Delta)$  can attack $\htt$ if and only if 
$\htt(g(\vx, \Delta))=\hbd(g(\vx, \Delta))\neq y.$ Furthermore,  under Assumption \ref{assm:S},  the poisoned sample $g(\vx, \Delta)$ is an adversarial example of Type \RNum{3}, called Shared Adversarial Example, if it can attack $\htt$.
\end{proposition}

Proposition~\ref{ass:share} suggests that the shared adversarial examples serve as better substitutes for poisoned samples than vanilla  adversarial examples. Denote the set of shared adversarial examples by $\Asha(\veps, \vtheta) = \{(\tilde{\vx}(\veps),y)| \hbd(\tilde{\vx}(\veps))=\htt(\tilde{\vx}(\veps)), \tilde{\vx}(\veps) \in \gA(\veps, \vtheta) \}$. % and its complementary $\Af(\veps, \vtheta) = \{\tilde{\vx}(\veps) \in \gA(\veps, \vtheta)| \hbd(\tilde{\vx}(\veps))\neq \htt(\tilde{\vx}(\veps))\}$. 
  Then, we propose the following mixed adversarial risk 
    \begin{equation}
    \label{eq::sha_risk}
    \begin{aligned}
    \gR_{mix}(\htt) = &\frac{1}{|\Dn|} \sum_{i=1}^N \max_{\veps_i \in \gS} \Big\{\underbrace{\ind(\vx_i\in \Ds, \tilde{\vx}_i(\veps_i) \in \Asha(\veps_i, \vtheta))}_{\text{shared adversarial examples on } \Ds}\\
    &+\underbrace{\ind(\vx_i\in\Df, \tilde{\vx}_i(\veps_i) \in \gA(\veps_i, \vtheta))}_{\text{vanilla  adversarial examples on } \Df}\Big\}
    \end{aligned}
    \end{equation}

Compared to vanilla  adversarial risk $\gR_{adv}$, the proposed mixed adversarial risk $\gR_{mix}$ focuses on the shared adversarial examples for samples in $\Ds$ while considering vanilla  adversarial examples for samples in $\Df$. When $\Ds=\Dn$, the mixed adversarial risk measures the shared adversarial risk on $\Dn$ and it is equivalent to $\gR_{adv}$ if $\Ds=\emptyset$. The following proposition describes the the gap between $\gR_{adv}$ and $\gR_{mix}$: 

\begin{proposition}
\label{pro:gap}
For a classifier $\htt$, we have 
$$\gR_{adv}(\htt) -  \gR_{mix}(\htt) \geq \frac{\sum_{i=1}^N \ind(\vx_i\in \Ds, \tilde{\vx}_i(\veps_i^*)\in \gA(\veps_i^*, \vtheta)\setminus\Asha(\veps_i^*,\theta))}{|\Dn|},$$
where $\veps^*_i$ the the solution to $(\ref{eq::sha_risk})$.
\end{proposition}

Then, we provide the following theorem  to establish the relation between backdoor risk and (shared) adversarial risk:

\begin{theorem}
Under Assumption \ref{assm:S}, for a classifier $\htt$, the following inequalities hold
$$\gR_{bd}(\htt) \leq  \gR_{mix}(\htt) \leq \gR_{adv}(\htt).$$
\end{theorem}

Finally, replacing $\gR_{bd}$ with $\gR_{mix}$ in Problem \ref{eq::trade}, we reach the following problem:

\begin{equation}
    \label{eq::final_risk}
    \min_{\vtheta} \gR_{cl}(\htt) + \lambda \gR_{mix}(\htt).
\end{equation}
By solving ($\ref{eq::final_risk}$), we seek  $\htt$ that either classifies the adversarial examples correctly i.e., $\htt(\tilde{\vx})=y$, or differently than $\hbd$ ,i.e., $\htt(\tilde{\vx})\neq \hbd(\tilde{\vx})$, while maintain a high accuracy on $\Db$. %We remark that compared with objective in \ref{eq::trade} which aims to achieve $\htt(\vx+\Delta)\neq \hat{y}$, the objective in $\ref{eq::final}$ further enforce $\htt(\vx+\Delta)= y$ implicitly, which improve its practicability. 


\subsection{Proposed method}
\label{sec::loss}
Since the target label $\hat{y}$ is not accessible and 0-1 loss is indifferentiable, we first discuss the relaxation of $\gR_{mix}$ and then replace 0-1 loss with proper surrogate loss functions in this section.

\paragraph{Relaxation.} In Section~\ref{sec::risk}, we focus on samples whose labels are not the targeted label. Since $\htt(g(\vx,\Delta))= \hat{y}$ is acceptable if the ground truth label of $\vx$ is $\hat{y}$, we first relax the condition that $y\neq \hat{y}$ in $\gR_{mix}$. Another limitation to $\gR_{mix}$ is the inaccessibility of $\Ds$ and $\Df$. Note that $\Df$ involves  samples in which planting a trigger cannot activate the backdoor in $\hbd$. Since a backdoored model usually has a high attack success rate (ASR) %and a poisoned sample that fails to attack $\hbd$ is unlikely to successfully attack $\htt$ in the purification process
, we relax the requirement of $\Ds$ and $\Df$ in $\gR_{mix}$. And we will show that such relaxation works even for $\hbd$ with a low ASR in the experiment section.  After relaxation, we reach the following shared adversarial risk on $\Db$: 
$$\gR_{sa}(\htt) = \frac{1}{N}\sum_{i=1}^N \max_{\veps_i\in \gS} \ind(\htt(\tilde{\vx}_i(\veps_i))\neq y_i, \htt(\tilde{\vx}_i(\veps_i))= \hbd(\tilde{\vx}_i(\veps_i))).$$

\paragraph{Surrogate loss.} After relaxation, we need to consider two indicators: 1) $\ind(\htt(\vx_i)\neq y_i)$; 2) $\ind(\htt(\tilde{\vx}_i(\veps_i))\neq y, \htt(\tilde{\vx}_i(\veps_i))= \hbd(\tilde{\vx}_i(\veps_i)))$.

The first indicator is for the clean accuracy, so we use the popular cross-entropy (CE) loss as the surrogate loss, i.e., $\ell_1(\vtheta,(\vx_i,y_i)) = \text{CE}(\vp(\vx_i,\vtheta),y_i)$.  For the second term which considers the shared adversarial risk, we choose different losses for the maximization step and minimization step, respectively.


\paragraph{Minimization step.} In the minimization step, we aim to reduce the shared adversarial risk. Since $\hbd(\tilde{\vx}_i(\veps_i))$ can be regarded as a surrogate for the target label and $\hbd$ is fixed, we use $\hbd(\tilde{\vx}_i(\veps_i)))$ as a hard label and choose  $$\ell_2(\vtheta,(\tilde{\vx}_i(\veps_i),y_i)) = - \ind\left( \tilde{y}_i\neq y_i\right)\log\left(1-\vp_{\tilde{y}_i}(\tilde{\vx}_i(\veps_i),\vtheta)\right),$$
where $\tilde{y}_i = \hbd(\tilde{\vx}_i(\veps_i))$.


\textbf{Maximization step.} In the maximization step, we aim to generate adversarial examples that mislead $\htt$ and $\hbd$ to the same label. To achieve this objective, a simple way is to perform a targeted adversarial attack on $\htt$ and $\hbd$ with random target labels and we left this method to Appendix. Another way is to perform an untargeted adversarial attack with regularization for shared adversarial perturbation. To do so, we first rewrite the second indicator as 
\begin{equation*}
  \ind(\htt(\tilde{\vx}_i(\veps_i))\neq y_i, \hbd(\tilde{\vx}_i(\veps_i))\neq y_i )\ind( \htt(\tilde{\vx}_i(\veps_i)) = \hbd(\tilde{\vx}_i(\veps_i))).  
\end{equation*}

From the above formulation, we can decompose the original  indicator into two components standing for fooling $\hbd$ and $\htt$ simultaneously and keeping the same predicted label for $\hbd$ and $\htt$. For the first component, we use CE as a surrogate loss, i.e., 
$$\ell_3(\vtheta,(\tilde{\vx}_i(\veps_i),y_i)) = \text{CE}(\vp(\tilde{\vx}_i(\veps_i),\vtheta),y_i)+ \text{CE}(\vp(\tilde{\vx}_i(\veps_i),\vtheta_{bd}),y_i).$$ 

Note that other loss functions for adversarial robustness can also be used here. For the second component, we measure the distance between $\vp(\tilde{\vx}_i(\veps_i),\vtheta)$ and $\vp(\tilde{\vx}_i(\veps_i),\vtheta_{bd})$ by Jensen-Shannon  divergence and design the following loss:
$$\ell_4(\vtheta,(\tilde{\vx}_i(\veps_i),y_i)) = \text{JS}(\vp(\tilde{\vx}_i(\veps_i),\vtheta_{bd}),\vp(\tilde{\vx}_i(\veps_i),\vtheta_{bd})).$$




% \paragraph{Inner Maximization} In inner maximization, we aim to find the CUP by solving problem \ref{eq::cup_risk}. So, we consider the surrogate loss functions for two term 1). $\ind(\htt(\tilde{\vx}_i(\veps_i))\neq y_i)$, and 2). $- \ind(\htt(\tilde{\vx}_i(\veps_i))\neq y_i, \htt(\tilde{\vx}_i(\veps_i)) \neq \hbd(\tilde{\vx}_i(\veps_i)))$. For the first term, we employ the commonly used CE loss. Since the second term aims to encourage $\htt(\tilde{\vx}_i(\veps_i))=\hbd(\tilde{\vx}_i(\veps_i))$ under that condition that $\htt(\tilde{\vx}_i(\veps_i))\neq y_i$, we regard $\htt(\tilde{\vx}_i(\veps_i))$ as hard label and use CE loss to replace the second term.

\paragraph{Overall objective.} Combine all the surrogate loss functions and we propose the following bi-level objective:
\begin{equation}
\label{eq::overall}
\begin{aligned}
    \min_{\vtheta} \quad &\frac{1}{N} \sum_{i=1}^N \{  \lambda_1 \ell_1(\vtheta,(\vx_i,y_i)) + \lambda_2  \ell_2(\vtheta,(\tilde{\vx}_i(\veps_i^*),y_i))\} \\
    \quad & \veps_i^* = \argmax_{\veps_i \in \gS} \lambda_3 \ell_3(\vtheta,(\tilde{\vx}_i(\veps_i),y_i)) +\lambda_4  \ell_4(\vtheta,(\tilde{\vx}_i(\veps_i),y_i)). 
\end{aligned}
\end{equation}

Since different surrogate losses have different scales and properties, we add a coefficient for each loss to control the tradeoff between different losses.

% \begin{equation}
% \resizebox{0.94\linewidth}{!}{$
% \begin{aligned}
%     \min_{\vtheta} \quad &\frac{1}{N} \sum_{i=1}^N \{\text{CE}(\vp(\vx_i,\theta),y_i) + \lambda_1 \text{BCE}(\vp(\tilde{\vx}_i(\veps^*),\theta),y_i) \\
%     & \quad \quad \quad- \lambda_2 \ind(\htt(\tilde{\vx}_i(\veps^*))=\hbd(\tilde{\vx}_i(\veps^*)))\log\left(1-\vp_{\htt(\tilde{\vx}_i(\veps^*))}(\tilde{\vx}_i(\veps^*),\theta)\right)\} \\
%     \mathrm{s.t.}
%     \quad & \veps^* = \argmax_{\veps\in \gS} \frac{1}{N} \sum_{i=1}^N \text{CE}(\vp(\tilde{\vx}_i(\veps_i),\theta),y_i) - \beta_1 \ind(\htt(\tilde{\vx}_i(\veps_i))\neq y_i)\text{CE}(\vp(\tilde{\vx}_i(\veps_i), \vtheta_{bd}), \htt(\tilde{\vx})). 
% \end{aligned}$}
% \end{equation}

% \paragraph{Adaptation to batch normalization } Batch normalization (BN) has been widely used in modern deep neural networks due to improved convergence. However, recent works show that it is difficult for BN to estimate the correct normalization statistics of a mixture of distributions of adversarial examples and clean examples \cite{XieY20,wang2022removing}. Such a problem is magnified when we adversarially fine-tune a model with a small set of samples and may destroy the generalization ability of the model due to biased BN statistics.  To address this problem, we propose to fix the BN statistic in the adversarial unlearning process and we will show that such operation benefits others adversarial-based methods in general.





==> backups/method_20230515.tex <==
In Section~\ref{sec::pre}, we first introduce notations, threat model, and defense goal to formulate the problem. By investigating the relationship between adversarial risk and backdoor risk, a new upper bound of backdoor risk is derived in Section~\ref{sec::risk}, from which a bi-level formulation is proposed in Section \ref{sec::loss}.


\subsection{Preliminary}
\label{sec::pre}

\paragraph{Notations.} 
% \red{[Mingda: Is it necessary to add this sentence?]} Let lowercase symbols and lowercase boldface symbols denote scalars and vectors, respectively.
Let uppercase calligraphic symbols denote sets/spaces and risks. We consider a $K$-class ($K\geq 2$) classification problem that aims to predict the label $y\in \gY$ of a given sample $\vx \in \gX$, where $\gY=[1, \cdots, K]$ is the set of labels and $\gX$ is the space of samples. Let $h_{\vtheta}:\gX\to \gY$ be a DNN classifier with model parameter $\vtheta$. We use $\gD$ to denote the set of data $(\vx,y)$. %\red{[Mingda: do you use this abbreviation in the passage?]} used 
For simplicity, we use $\vx\in \gD$ as a abbreviation for $(\vx,y)\in \gD$. Then, for a sample $\vx\in \gD$,  its predicted label is
\begin{equation}
    \htt(\vx) = \argmax_{k=1,\cdots, K} \vp_k(\vx,\vtheta), 
\end{equation}
where $\vp_k(\vx,\vtheta)$ is the (softmax) probability of $\vx$ belonging to class $k$. 

\paragraph{Threat model.}
Let $\gV$ be the set of triggers and define $g:\gX\times \gV \to \gX$ as the generating function for poisoned samples. Then, given a trigger $\Delta \in \gV$ and a sample $\vx\in \gX$, one can generate a poisoned sample $g(\vx,\Delta)$. For simplicity, we only consider all to one case, \ie, there is only one trigger $\Delta$ and one target label $\hat{y}$. The all to all case and multi-trigger case are left in the \app. We assume that the attacker has access to manipulate the dataset and/or control the training process such that the trained model classifies the samples with pre-defined trigger $\Delta$ to the target labels $\hat{y}$ while classifying clean samples normally.  In addition, we define the poisoning ratio as the proportion of poisoned samples in the training dataset. 

\paragraph{Defense goal.}
We consider a scenario where a defender is given a poisoned  model with parameter $\theta_{bd}$ and a small set of \textit{clean} data $\Db=\{(\vx_i,y_i)\}_{i=1}^N$. Since we are mainly interested in samples whose labels are not the target label, we further define the set of non-target samples as $\Dn = \{(\vx,y) |(\vx,y) \in \Db, y\neq \hat{y}\}$. Note that the size of $\Db$ is small and the defender cannot train a new model from scratch using only $\Db$. The defender's goal is to purify the model so that the clean performance is maintained and the backdoor effect is removed or mitigated. We assume that the defender cannot access the trigger  $\Delta$ or the target label $\hat{y}$.

\paragraph{Problem formulation.}
Using the $0$-$1$ loss \cite{ wang2020improving, zhang2019theoretically}, the classification risk $\gR_{cl}$ and the backdoor risk $\gR_{bd}$ with respect to classifier $\htt$ on $\Db$ can be defined as:
\begin{align}
    \label{eq::risk}
    \gR_{cl}(\htt) = \frac{1}{N}\sum_{i=1}^N \ind(\htt(\vx_i)\neq y_i), \quad
    \gR_{bd}(\htt) = \frac{\sum_{i=1}^N \ind(\htt(g(\vx_i,\Delta))=\hat{y}, \vx_i\in \Dn)}{|\Dn|}%{\sum_{j=1}^N \ind(y_j\neq \hat{y})},
\end{align}
where $\ind$ is the indicator function and $|\cdot|$ denotes the cardinality of a set.

In (\ref{eq::risk}), the classification risk concerns whether a clean sample is  correctly classified, while the backdoor risk measures the risk of classifying a poisoned sample from $\Dn$ to target class $\hat{y}$. 

% Since the backdoor risk only focuses on breaking the relationship between trigger $\Delta$ and target label $\hat{y}$, merely minimizing $\gR_{bd}(\htt)$ may lead to an unacceptable increase of $\gR_{cl}(\htt)$. 
In this paper, we consider the following problem for purifying a poisoned model:
\begin{equation}
    \label{eq::trade}
    \min_{\vtheta} \gR_{cl}(\htt) + \lambda \gR_{bd}(\htt),
\end{equation}
where $\lambda$ is a hyper-parameter to control the tradeoff between classification risk and backdoor risk.

\subsection{Connection between backdoor risk and adversarial risk}
\label{sec::risk}
%Since neither the trigger $\Delta$ nor target label $\hat{y}$ is accessible to the defender, directly minimizing (\ref{eq::trade}) is impractical. 
Since directly minimizing (\ref{eq::trade}) is impractical, a natural choice is to replace $\gR_{bd}$ with a proper upper bound. Therefore, we delve deeper for adversarial risk as an upper bound of backdoor risk.

Let $\gS$ be a set of perturbations. Given a sample $\vx$ and an adversarial perturbation $\veps$, an adversarial example $\tilde{\vx}_{\veps}$ can be generated by $\tilde{\vx}_{\veps} = \vx+\veps$. We define the set of adversarial example-label pair to $\htt$ generated by perturbation $\veps$ and dataset $\Db$ by
$\gA_{\veps,\vtheta}=\{(\tilde{\vx}_{\veps},y)|\htt(\tilde{\vx}_{\veps})\neq y, (\vx,y)\in \Db\}$ and abbreviate $(\tilde{\vx}_{\veps},y) \in \gA_{\veps,\vtheta}$ by $\tilde{\vx}_{\veps} \in \gA_{\veps,\vtheta}$. Then, the adversarial risk for $\htt$ on $\Dn$ can be defined as
\begin{equation}
    \label{eq::ae_risk}
    \gR_{adv}(\htt) = \frac{\sum_{i=1}^N \max_{\veps_i \in \gS}\ind(\tilde{\vx}_{i, \veps_i} \in \gA_{\veps_i,\vtheta}, \vx_i\in\Dn)}{|\Dn|}.
\end{equation}


To bridge the adversarial examples and poison samples, we provide the following assumption:
\begin{assumption}  
\label{assm:S}
Assume that $g(\vx,\Delta) - \vx \in \gS$ for  $\forall \vx \in \Db$.
\end{assumption}

Assumption \ref{assm:S} ensures that there exists $\veps \in \gS$ such that $\vx+\veps = g(\vx,\Delta)$. As poisoned samples are required to be stealthy and imperceptible to humans \cite{nguyen2021wanet, wubackdoorbench,  zeng2021rethinking}, Assumption \ref{assm:S} is quite mild. For example, an $L_p$ ball with radius $\rho$, \ie, $\gS=\{\veps |\|\veps\|_p\leq \rho \}$, is sufficient to satisfy Assumption \ref{assm:S} with proper $p$ and $\rho$.

Then, we reach the first upper bound of backdoor risk:
\begin{proposition}
    Under Assumption~\ref{assm:S}, $\gR_{adv}$ serves as an upper bound of $\gR_{bd}$, \ie, $\gR_{bd}\leq \gR_{adv}$.
\end{proposition}

\begin{wrapfigure}{r}{0.5\textwidth}
  \begin{center}
    \includegraphics[width=0.48\textwidth]{images/at.pdf}
  \end{center}
  \caption{Example of purifying poisoned model using adversarial training on Tiny ImageNet  \cite{le2015tiny}.}
  \label{gap}
  \vspace{-0.3in}
\end{wrapfigure}

Although $\gR_{adv}$ seems to be a promising surrogate for $\gR_{bd}$, it neglects some essential connections between adversarial examples and poisoned samples, resulting in a significant gap between adversarial risk and backdoor risk, as shown in Figure \ref{gap}. Such a gap also leads to a fluctuating learning curve for backdoor risk and an avoidable  drop in accuracy in the backdoor mitigation process.

Therefore, we seek to construct a tighter  upper for $\gR_{bd}$. A key insight is that not all adversarial examples contribute to backdoor mitigation. To further identify AEs important for mitigating backdoors, we leverage   the information from the poisoned model to categorize the adversarial examples into three types, as shown in Table~\ref{tab:AE}.

% \begin{table}[h]
%   \caption{Categories of adversarial examples to $\htt$.}
%   \label{tab:AE}
%   \centering
%   \begin{tabular}{lll}
%     \toprule
%     \cmidrule(r){1-3}
%     Type     & Description     & Definition \\
%     \midrule
%     % \RNum{1}       & Mislead $\hbd$ only   & $\hbd(\tilde{\vx}_{\veps})\neq y, \htt(\tilde{\vx}_{\veps}) = y$     \\
%     \RNum{1}       & Mislead $\htt$ only & $\hbd(\tilde{\vx}_{\veps}) = y$     \\
%     \RNum{2}      & Mislead $\hbd$ and $\htt$ to the same class       & $\hbd(\tilde{\vx}_{\veps}) = \htt(\tilde{\vx}_{\veps})$ \\
%     \RNum{3}       & Mislead $\hbd$ and $\htt$ to different classes  & $\hbd(\tilde{\vx}_{\veps}) \neq \htt(\tilde{\vx}_{\veps}), \hbd(\tilde{\vx}_{\veps}) \neq y$     \\
%     \bottomrule
%   \end{tabular}
% \end{table}



\begin{table}[h]
  \caption{Different types of adversarial examples to $\htt$. }
  \label{tab:AE}
  \centering
    \scalebox{0.95}{
  \begin{tabular}{lll}
    \toprule
    \cmidrule(r){1-3}
    Type     & Description     & Definition \\
    \midrule
    % \RNum{1}       & Mislead $\hbd$ only   & $\hbd(\tilde{\vx}_{\veps})\neq y, \htt(\tilde{\vx}_{\veps}) = y$     \\
    \RNum{1}      & Mislead $\hbd$ and $\htt$ to the same class       & $\hbd(\tilde{\vx}_{\veps}) = \htt(\tilde{\vx}_{\veps}) \neq y$ \\
    \RNum{2}       & Mislead $\htt$, but bot mislead $\hbd$ & $\hbd(\tilde{\vx}_{\veps}) \neq \htt(\tilde{\vx}_{\veps}), \hbd(\tilde{\vx}_{\veps}) = y$     \\
    \RNum{3}       & Mislead $\hbd$ and $\htt$ to different classes  & $\hbd(\tilde{\vx}_{\veps}) \neq \htt(\tilde{\vx}_{\veps}), \hbd(\tilde{\vx}_{\veps}) \neq y, \htt(\tilde{\vx}_{\veps}) \neq y$     \\
    \bottomrule
  \end{tabular}}
\end{table}


\begin{figure}[h]
    \centering
    \includegraphics[width = 0.9\linewidth]{images/venn_4.pdf}
    \caption{A schematic of the relationship between adversarial example, shared adversarial example and poisoned samples. The adversarial examples for $\hbd$ and $\htt$ are shown in blue and orange, respectively. The poisoned samples are indicated by red. By decreasing the shared adversarial examples between $\hbd$ and $\htt$ (from $(a)$ to $(b)$), the backdoor risk can be mitigated.}
    \label{fig::cup}
\end{figure}


Let $\Ds = \{(\vx,y)|\hbd(g(\vx, \Delta))=\hat{y}, \vx\in \Dn\}$ be the subset of samples in $\Dn$ on which planting a trigger can successfully activate the backdoor in $\hbd$. As illustrated in Figure ~\ref{fig::cup}, the following proposition reveals a deeper connection between adversarial examples and poisoned samples.

\begin{proposition} 
\label{ass:share}
For $\forall (\vx,y) \in \Ds$, the poisoned sample $g(\vx, \Delta)$  can attack $\htt$ if and only if 
$\htt(g(\vx, \Delta))=\hbd(g(\vx, \Delta))\neq y.$ Furthermore,  under Assumption \ref{assm:S},  the poisoned sample $g(\vx, \Delta)$ is an adversarial example of Type \RNum{1}, called Shared Adversarial Example, if it can attack $\htt$.
\end{proposition}

 
Then, the adversarial risk $\gR_{adv}$ can be decomposed to three components as below:
\begin{equation}
\label{eq::decom}
\begin{aligned}
    &\gR_{adv}(\htt) = \frac{1}{|\Dn|} \sum_{i=1}^N \max_{\veps_i \in \gS} \Big\{\underbrace{\ind(\vx_i\in \Ds)\ind(\htt(\tilde{\vx}_{i, \veps_i})=\hbd(\tilde{\vx}_{i, \veps_i}), \tilde{\vx}_{i, \veps_i} \in \gA_{\veps_i,\vtheta})}_{\text{Type \RNum{1} adversarial examples on } \Ds} \\
    &+ \underbrace{\ind(\vx_i\in \Ds)\ind(\htt(\tilde{\vx}_{i, \veps_i})\neq\hbd(\tilde{\vx}_{i, \veps_i}), \tilde{\vx}_{i, \veps_i} \in \gA_{\veps_i,\vtheta})}_{\text{Type \RNum{2} or \RNum{3} adversarial examples on } \Ds} + \underbrace{\ind(\vx_i\in \Dn\setminus\Ds, \tilde{\vx}_{i, \veps_i} \in \gA_{\veps_i,\vtheta})}_{\text{vanilla  adversarial examples on } \Dn\setminus\Ds}\Big\}
\end{aligned}   
\end{equation}


Proposition~\ref{ass:share} implies  that the first component in $(\ref{eq::decom})$ is essential  for mitigating backdoors as it captures the shared adversarial examples between the poisoned model $\hbd$ and the fine-tuned model $\htt$. The second component is insignificant since adversarial examples of Type \RNum{2} and \RNum{3} are either not poisoned samples or ineffective to attack $\htt$. The third component protects the samples that are resistant to triggers from being attacked in the mitigation process.
% 

By removing the second component in $(\ref{eq::decom})$, we propose the following sub-adversarial risk
\begin{equation}
\label{eq::sha_risk}
\begin{aligned}
    \gR_{sub}(\htt) = &\frac{1}{|\Dn|} \sum_{i=1}^N \max_{\veps_i \in \gS} \Big\{\ind(\vx_i\in \Ds)\ind(\htt(\tilde{\vx}_{i, \veps_i})=\hbd(\tilde{\vx}_{i, \veps_i}), \tilde{\vx}_{i, \veps_i} \in \gA_{\veps_i,\vtheta}) \\
    & + \ind(\vx_i\in \Dn\setminus\Ds, \tilde{\vx}_{i, \veps_i} \in \gA_{\veps_i,\vtheta})\Big\}
\end{aligned}   
\end{equation}

Compared to vanilla  adversarial risk $\gR_{adv}$, the proposed sub-adversarial risk $\gR_{sub}$ focuses on the shared adversarial examples for samples in $\Ds$ while considering vanilla  adversarial examples for samples in $\Dn\setminus\Ds$. When $\Ds=\Dn$, the sub-adversarial risk measures the shared adversarial risk on $\Dn$ and it is equivalent to $\gR_{adv}$ if $\Ds=\emptyset$. 

%The following proposition describes the the gap between $\gR_{adv}$ and $\gR_{sub}$: 
% \begin{proposition}
% \label{pro:gap}
% For a classifier $\htt$, we have 
% $$\gR_{adv}(\htt) -  \gR_{sub}(\htt) \geq \frac{\sum_{i=1}^N \ind(\vx_i\in \Ds, \tilde{\vx}_i(\veps_i^*)\in \gA(\veps_i^*, \vtheta)\setminus\Asha(\veps_i^*,\theta))}{|\Dn|},$$
% where $\veps^*_i$ the the solution to $(\ref{eq::sha_risk})$.
% \end{proposition}

Then, we provide the following theorem  to establish the relation between backdoor risk and (sub) adversarial risk:

\begin{theorem}
Under Assumption \ref{assm:S}, for a classifier $\htt$, the following inequalities hold
$$\gR_{bd}(\htt) \leq  \gR_{sub}(\htt) \leq \gR_{adv}(\htt).$$
\end{theorem}

Therefore, $\gR_{sub}$ is a tighter upper bound for $\gR_{bd}$ compared with $\gR_{adv}$. Due to space constraints, the proofs, detailed discussion and extensions are left to the \app.

\subsection{Proposed method}
\label{sec::loss}
Since the target label $\hat{y}$ is unavailable and 0-1 loss is non-differentiable, we first discuss the relaxation of $\gR_{sub}$ and then replace 0-1 loss with suitable surrogate loss functions in this section.

\paragraph{Relaxation.}  One limitation of $\gR_{sub}$ is the inaccessibility of $\Ds$. Since a poisoned model usually has a high attack success rate (ASR), we first relax the requirement for $\Ds$ and focus on shared adversarial examples for all samples in $\Dn$. We will show that such relaxation works even for $\hbd$ with a low ASR in the experiment section. Since $\hat{y}$ is unavailable, we also replace $\Dn$ by $\Db$ in the sub-adversarial risk. Since $g(\vx,\Delta)$ is not harmful if the ground truth label of $\vx$ is $\hat{y}$ and modern classification task usually has a large number of classes, this relaxation has little negative influence for mitigating backdoor risk. After relaxation, we reach the following shared adversarial risk on $\Db$: 
$$\gR_{share}(\htt) = \frac{1}{N}\sum_{i=1}^N \max_{\veps_i\in \gS} \ind(\htt(\tilde{\vx}_{i, \veps_i})\neq y_i, \htt(\tilde{\vx}_{i, \veps_i})= \hbd(\tilde{\vx}_{i, \veps_i})).$$

After replacing $\gR_{bd}$ with $\gR_{share}$ in Problem \ref{eq::trade}, we reach the following problem:

\begin{equation}
    \label{eq::final_risk}
    \min_{\vtheta} \gR_{cl}(\htt) + \lambda \gR_{share}(\htt).
\end{equation}
By solving ($\ref{eq::final_risk}$), we seek  $\htt$ that either classifies the adversarial examples correctly \ie, $\htt(\tilde{\vx}_{\veps})=y$, or differently to $\hbd$ ,\ie, $\htt(\tilde{\vx}_{\veps})\neq \hbd(\tilde{\vx}_{\veps})$, while maintain a high accuracy on $\Db$. %We remark that compared with objective in \ref{eq::trade} which aims to achieve $\htt(\vx+\Delta)\neq \hat{y}$, the objective in $\ref{eq::final}$ further enforce $\htt(\vx+\Delta)= y$ implicitly, which improve its practicability. 

\paragraph{Approximation.} After relaxation, we need to approximate two indicators: 1) $\ind(\htt(\vx_i)\neq y_i)$; 2) $\ind(\htt(\tilde{\vx}_{i, \veps_i})\neq y, \htt(\tilde{\vx}_{i, \veps_i})= \hbd(\tilde{\vx}_{i, \veps_i}))$.

The first indicator is for the clean accuracy, so we use the popular cross-entropy (CE) loss as the surrogate loss, \ie, $L_{cl}(\vtheta,(\vx_i,y_i)) = \text{CE}(\vp(\vx_i,\vtheta),y_i)$.  For the second term which considers the shared adversarial risk, we choose different losses for the inner minimization and outer maximization, respectively.


\textbf{Outer minimization.} In outer minimization, we aim to reduce the shared adversarial risk  (SAR) by unlearning the shared adversarial examples. Since $\hbd(\tilde{\vx}_{i, \veps_i})$ can be regarded as a surrogate for the target label and $\hbd$ is fixed, we use $\hbd(\tilde{\vx}_{i, \veps_i}))$ as a hard label and choose  $$L_{sar}(\vtheta,(\tilde{\vx}_{i, \veps_i},y_i)) = - \ind\left( \tilde{y}_i\neq y_i\right)\log\left(1-\vp_{\tilde{y}_i}(\tilde{\vx}_{i, \veps_i},\vtheta)\right),$$
where $\tilde{y}_i = \hbd(\tilde{\vx}_{i, \veps_i})$.

\textbf{Inner maximization.} In inner minimization, we aim to generate adversarial examples that mislead $\htt$ and $\hbd$ to the same label.  To achieve this objective, we perform an untargeted adversarial attack with regularization for shared adversarial examples. To do so, we first rewrite the second indicator as 
\begin{equation*}
  \ind(\htt(\tilde{\vx}_{i, \veps_i})\neq y_i, \hbd(\tilde{\vx}_{i, \veps_i})\neq y_i )\ind( \htt(\tilde{\vx}_{i, \veps_i}) = \hbd(\tilde{\vx}_{i, \veps_i})).  
\end{equation*}

From the above formulation, we can decompose the original  indicator into two components standing for fooling $\hbd$ and $\htt$ simultaneously and keeping the same predicted label for $\hbd$ and $\htt$. For the first component, we use CE as a surrogate loss, \ie, 
$$L_{adv}(\vtheta,(\tilde{\vx}_{i, \veps_i},y_i)) = \text{CE}(\vp(\tilde{\vx}_{i, \veps_i},\vtheta),y_i)+ \text{CE}(\vp(\tilde{\vx}_{i, \veps_i},\vtheta_{bd}),y_i).$$ 

For the second component, we measure the distance between $\vp(\tilde{\vx}_{i, \veps_i},\vtheta)$ and $\vp(\tilde{\vx}_{i, \veps_i},\vtheta_{bd})$ by Jensen-Shannon  divergence \cite{fuglede2004jensen} and design the following loss:
$$L_{share}(\vtheta,(\tilde{\vx}_{i, \veps_i},y_i)) = - \text{JS}(\vp(\tilde{\vx}_{i, \veps_i},\vtheta),\vp(\tilde{\vx}_{i, \veps_i},\vtheta_{bd})).$$


\textbf{Overall objective.} Combine all the surrogate loss functions and we propose the following bi-level objective, called Shared Adversarial Unlearning (SAU):
\begin{equation}
\label{eq::overall}
\begin{aligned}
    \min_{\vtheta} \quad &\frac{1}{N} \sum_{i=1}^N \left\{  \lambda_1 L_{cl}(\vtheta,(\vx_i,y_i)) + \lambda_2  L_{sar}(\vtheta,(\tilde{\vx}_{i,\veps_i^*},y_i))\right\} \\
    \mathrm{s.t.} \quad & \veps_i^* = \argmax_{\veps_i \in \gS} \lambda_3 L_{adv}(\vtheta,(\tilde{\vx}_{i, \veps_i},y_i)) +\lambda_4  L_{share}(\vtheta,(\tilde{\vx}_{i, \veps_i},y_i)). 
\end{aligned}
\end{equation}

Since different surrogate losses have different scales and properties, we add a coefficient for each loss to control the trade-off between them.





==> packages/defs.tex <==
\newcommand{\ones}{\mathbf 1}
\newcommand{\reals}{{\mathbb{R}}}
\newcommand{\integers}{{\mbox{\bf Z}}}
\newcommand{\symm}{{\mbox{\bf S}}}  % symmetric matrices

\newcommand{\nullspace}{{\mathcal N}}
\newcommand{\range}{{\mathcal R}}
\newcommand{\Rank}{\mathop{\bf Rank}}
\newcommand{\Tr}{\mathop{\bf Tr}}
\newcommand{\diag}{\mathop{\bf diag}}
\newcommand{\card}{\mathop{\bf card}}
\newcommand{\rank}{\mathop{\bf rank}}
\newcommand{\conv}{\mathop{\bf conv}}
\newcommand{\prox}{\mathbf{prox}}


\newcommand{\xmark}{\text{\ding{55}}}
\newcommand{\cmark}{\text{\ding{51}}}

\newcommand{\smallfont}[1]{{\small#1}}
\newcommand{\dquote}[1]{``#1"}
% color
\newcommand{\cred}[1]{{\color{red}#1}}
\newcommand{\cblue}[1]{{\color{blue}#1}}
\newcommand{\blue}[1]{\textcolor[rgb]{0.00,0.00,1.00}{#1}}
\newcommand{\green}[1]{\textcolor[rgb]{0.00,0.50,0.00}{#1}}

\newcommand{\Expect}{\mathop{\bf E{}}}
\newcommand{\Prob}{\mathop{\bf Prob}}
\newcommand{\Co}{{\mathop {\bf Co}}} % convex hull
\newcommand{\dist}{\mathop{\bf dist{}}}
\newcommand{\epi}{\mathop{\bf epi}} % epigraph
\newcommand{\Vol}{\mathop{\bf vol}}
\newcommand{\dom}{\mathop{\bf dom}} % domain
\newcommand{\intr}{\mathop{\bf int}}
\newcommand{\sign}{\mathop{\bf sign}}
\newcommand{\avg}{\operatorname{avg}}

\newcommand{\cf}{{\it cf.}}
\newcommand{\eg}{{\it e.g.}}
\newcommand{\ie}{{\it i.e.}}
\newcommand{\etc}{{\it etc.}}

\newcommand{\tra}{\mathrm{tr}}


==> packages/header.tex <==
% % \usepackage[utf8]{inputenc} % allow utf-8 input
% %\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% %\usepackage{hyperref}       % hyperlinks
% \usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypogrhy
% \usepackage{natbib}
% \usepackage{enumerate}
% %\usepackage{enumitem}
% \usepackage{hhline}
% \usepackage{makecell}
% \usepackage{pifont}
% \usepackage{tcolorbox}
% \usepackage{color}
% \usepackage{cancel}

% % use Times
% %\usepackage{times}
% % For figures
% \usepackage{graphicx} % more modern
% %\usepackage{epsfig} % less modern
% %\usepackage{subfigure}
% \usepackage{caption}
% \usepackage{subcaption}
% % For citations
% \usepackage{amsmath}
% \usepackage{amsthm}
% \usepackage{amssymb}
% \usepackage{tikz}
% \usepackage{xcolor}
% \usetikzlibrary{arrows}

% \allowdisplaybreaks

% %for fonts
% \usepackage{mathrsfs}

% % For algorithms
% \usepackage{algorithm}
% \usepackage{algorithmic}
% % \usepackage[noend]{algpseudocode}
% \usepackage{hyperref}
% \usepackage{bm}
% %\usepackage{todonotes}


% %For theorems
% \allowdisplaybreaks

% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}

% %for convinience
% \newcommand{\RR}{\mathbb{R}}
% \newcommand{\vct}{\boldsymbol }
% %\newcommand{\mat}{\mathbf}
% \newcommand{\rnd}{\mathsf}
% \newcommand{\ud}{\mathrm d}
% \newcommand{\nml}{\mathcal{N}}
% \newcommand{\loss}{\mathcal{L}}
% \newcommand{\hinge}{\mathcal{R}}
% \newcommand{\kl}{\mathrm{KL}}
% \newcommand{\cov}{\mathrm{cov}}
% \newcommand{\dir}{\mathrm{Dir}}
% \newcommand{\mult}{\mathrm{Mult}}
% \newcommand{\err}{\mathrm{err}}
% \newcommand{\sgn}{\mathrm{sgn}}
% %\renewcommand{\span}{\mathrm{span}}
% % \newcommand{\argmin}{\mathrm{argmin}}
% % \newcommand{\argmax}{\mathrm{argmax}}
% \newcommand{\poly}{\mathrm{poly}}
% % \newcommand{\rank}{\mathrm{rank}}
% % \newcommand{\conv}{\mathrm{conv}}
% %\newcommand{\E}{\mathbb{E}}
% % \newcommand{\diag}{\mat{diag}}
% \newcommand{\acc}{\mathrm{acc}}

% \newcommand{\leftabs}{\left\vert}
% \newcommand{\rightabs}{\right\vert}
% \newcommand{\leftnorm}{\left\Vert}
% \newcommand{\rightnorm}{\right\Vert}

% \newcommand{\aff}{\mathrm{aff}}
% % \newcommand{\range}{\mathrm{Range}}
% \newcommand{\Sgn}{\mathrm{sign}}

% \newcommand{\hit}{\mathrm{hit}}
% \newcommand{\cross}{\mathrm{cross}}
% \newcommand{\Left}{\mathrm{left}}
% \newcommand{\Right}{\mathrm{right}}
% \newcommand{\Mid}{\mathrm{mid}}
% \newcommand{\bern}{\mathrm{Bernoulli}}
% \newcommand{\ols}{\mathrm{ols}}
% \newcommand{\tr}{\mathrm{tr}}
% \newcommand{\opt}{\mathrm{opt}}
% %\newcommand{\ridge}{\mathrm{ridge}}
% \newcommand{\unif}{\mathrm{unif}}
% \newcommand{\Image}{\mathrm{im}}
% \newcommand{\Kernel}{\mathrm{ker}}
% \newcommand{\supp}{\mathrm{supp}}
% \newcommand{\pred}{\mathrm{pred}}
% \newcommand{\distequal}{\stackrel{\mathbf{P}}{=}}
% %\newcommand{\gege}{\textcircled{1}}
% \newcommand{\gege}{{A(\vect{w},\vect{w}_*)}}
% \newcommand{\gele}{{A(\vect{w},-\vect{w}_*)}}
% \newcommand{\lele}{{A(-\vect{w},-\vect{w}_*)}}
% \newcommand{\lege}{{A(-\vect{w},\vect{w}_*)}}
% \newcommand{\firstlayer}{\mathbf{W}}
% \newcommand{\firstlayerWN}{v}
% \newcommand{\secondlayer}{a}
% \newcommand{\inputvar}{\vect{x}}
% \newcommand{\anglemat}{\mathbf{\Phi}}
% \newcommand{\holder}{H\"{o}lder }
% \newcommand{\real}{\mathbb{R}}
% \newcommand{\approxerr}{\delta}

% \def\R{\mathbb{R}}
% \def\Z{\mathbb{Z}}
% \def\cA{\mathcal{A}}
% \def\cB{\mathcal{B}}
% \def\cD{\mathcal{D}}
% \def\cE{\mathcal{E}}
% \def\cF{\mathcal{F}}
% \def\cG{\mathcal{G}}
% \def\cH{\mathcal{H}}
% \def\cS{\mathcal{S}}
% \def\cI{\mathcal{I}}
% \def\cL{\mathcal{L}}
% \def\cM{\mathcal{M}}
% \def\cN{\mathcal{N}}
% \def\cP{\mathcal{P}}
% \def\cS{\mathcal{S}}
% \def\cT{\mathcal{T}}
% \def\cV{\mathcal{V}}
% \def\cW{\mathcal{W}}
% \def\cZ{\mathcal{Z}}
% \def\SS{\mathbb{S}}
% \def\NN{\mathbb{N}}
% \def\bP{\mathbf{P}}
% \def\TV{\mathrm{TV}}
% \def\MSE{\mathrm{MSE}}

% \def\vw{\mathbf{w}}
% \def\va{\mathbf{a}}
% \def\vZ{\mathbf{Z}}

% \newcommand{\mat}[1]{#1}
% \newcommand{\vect}[1]{#1}
% \newcommand{\norm}[1]{\left\|#1\right\|}
% \newcommand{\normop}[1]{\left\|#1\right\|_{\mathrm{op}}}
% \newcommand{\simplex}{\triangle}
% \newcommand{\abs}[1]{\left|#1\right|}
% \newcommand{\expect}{\mathbb{E}}
% \newcommand{\prob}{\mathbb{P}}
% % \newcommand{\prox}[2]{\textbf{Prox}_{#1}\left\{#2\right\}}
% \newcommand{\event}[1]{\mathscr{#1}}
% \newcommand{\set}[1]{#1}
% \newcommand{\diff}{\text{d}}
% \newcommand{\difference}{\triangle}
% \newcommand{\inputdist}{\mathcal{Z}}
% \newcommand{\indict}{\mathbb{I}}
% \newcommand{\rotmat}{\mathbf{R}}
% \newcommand{\normalize}[1]{\overline{#1}}
% \newcommand{\vectorize}[1]{\text{vec}\left(#1\right)}
% \newcommand{\vclass}{\mathcal{G}}
% \newcommand{\pclass}{\Pi}
% \newcommand{\qclass}{\mathcal{Q}}
% \newcommand{\rclass}{\mathcal{R}}
% \newcommand{\classComplexity}[2]{N_{class}(#1,#2)}
% \newcommand{\cclass}{\mathcal{F}}
% \newcommand{\gclass}{\mathcal{G}}
% \newcommand{\pthres}{p_{thres}}
% \newcommand{\ethres}{\epsilon_{thres}}
% \newcommand{\eclass}{\epsilon_{class}}
% \newcommand{\states}{\mathcal{S}}
% \newcommand{\trans}{P}
% \newcommand{\lowprobstate}{\psi}
% \newcommand{\actions}{\mathcal{A}}
% \newcommand{\contexts}{\mathcal{X}}
% \newcommand{\edges}{\mathcal{E}}
% \newcommand{\variance}{\text{Var}}
% \newcommand{\params}{\vect{w}}

% \newcommand{\relu}[1]{\sigma\left(#1\right)}
% \newcommand{\reluder}[1]{\sigma'\left(#1\right)}
% \newcommand{\act}[1]{\sigma\left(#1\right)}

\newtheorem{thm}{Theorem}
% \newtheorem{thm}{Theorem}
\newtheorem{lem}{Lemma}
% Thm -> corollary 
\newtheorem{cor}{Corollary}
\newtheorem{prop}{Proposition}
\newtheorem{asmp}{Assumption}
\newtheorem{defn}{Definition}
\newtheorem{oracle}{Oracle}
% \newtheorem{fact}{Fact}[section]
\newtheorem{conj}{Conjecture}
\newtheorem{rem}{Remark}
% \newtheorem{example}{Example}[section]
\newtheorem{condition}{Condition}



==> tables/gtsrb_preactresnet18_0_05.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h]
\centering
\caption{\textbf{GTSRB}, PREACTRESNET18, 5.0\%}
\label{gtsrb_preactresnet18_05}
%%% Caption here
\setlength{\tabcolsep}{3pt} % Default value: 6pt
% \renewcommand{\arraystretch}{1.5} % Default value: 1
\scalebox{0.72}{
\begin{tabular}{c|cccc|cccc|cccc|cccc}
\toprule
Defense & \multicolumn{4}{c|}{No Defense}    & \multicolumn{4}{c|}{ANP \cite{wu2021adversarial}}    & \multicolumn{4}{c|}{FP \cite{liu2018fine}}& \multicolumn{4}{c}{NC \cite{wang2019neural}}   \\ \midrule
Attack  & \multicolumn{1}{c}{ACC} & \multicolumn{1}{c}{ASR} & \multicolumn{1}{c}{R-ACC} & \multicolumn{1}{c|}{DER}& \multicolumn{1}{c}{ACC}  & \multicolumn{1}{c}{ASR} & \multicolumn{1}{c}{R-ACC} & \multicolumn{1}{c|}{DER}  & \multicolumn{1}{c}{ACC}         & \multicolumn{1}{c}{ASR}  & \multicolumn{1}{c}{R-ACC}& \multicolumn{1}{c|}{DER}  & \multicolumn{1}{c}{ACC}  & \multicolumn{1}{c}{ASR} & \multicolumn{1}{c}{R-ACC}& \multicolumn{1}{c}{DER}  \\
\midrule
BadNets \cite{gu2019badnets} & $97.3$& $57.95$& $6.89$&  N/A & $96.18$& $3.49$& $93.41$& $76.67$& $\underline{97.86}$& $2.11$& $92.42$& $\underline{77.92}$& $97.09$& $\textbf{0.00}$& $\textbf{97.11}$& $\textbf{78.87}$\\
Blended \cite{chen2017targeted} & $98.84$& $99.93$& $0.04$&  N/A & $98.69$& $99.98$& $0.02$& $49.92$& $\underline{98.75}$& $99.93$& $0.06$& $49.95$& $96.64$& $\textbf{3.14}$& $\textbf{58.33}$& $\textbf{97.29}$\\
Input-Aware \cite{nguyen2020input} & $97.04$& $93.17$& $6.76$&  N/A & $\textbf{nan}$& $\textbf{nan}$& $\textbf{nan}$& $50.00$& $98.23$& $11.42$& $85.97$& $\textbf{90.88}$& $97.04$& $93.17$& $6.76$& $50.00$\\
LF \cite{zeng2021rethinking} & $97.49$& $98.62$& $1.18$&  N/A & $\textbf{97.93}$& $85.77$& $12.55$& $56.43$& $97.70$& $98.03$& $1.44$& $50.30$& $97.77$& $\textbf{0.09}$& $\textbf{90.03}$& $\textbf{99.27}$\\
SSBA \cite{li2021invisible} & $98.11$& $99.34$& $0.63$&  N/A & $97.95$& $98.38$& $1.33$& $50.40$& $\textbf{98.12}$& $99.12$& $0.74$& $50.11$& $97.03$& $\underline{0.33}$& $\textbf{89.04}$& $\textbf{98.96}$\\
WaNet \cite{nguyen2021wanet} & $97.42$& $92.85$& $6.84$&  N/A & $97.74$& $\textbf{0.02}$& $\underline{97.69}$& $\textbf{96.42}$& $98.00$& $12.24$& $12.31$& $90.31$& $97.42$& $92.85$& $6.84$& $50.00$\\
Average & $97.7$& $90.31$& $3.72$&  N/A & $97.70$& $57.53$& $41.00$& $61.41$& $\underline{98.11}$& $53.81$& $32.16$& $65.64$& $97.16$& $31.60$& $\underline{58.02}$& $\underline{74.91}$\\

\toprule

\toprule
Defense & \multicolumn{4}{c|}{NAD \cite{li2021neural}}  & \multicolumn{4}{c|}{EP \cite{zheng2022preactivation}} & \multicolumn{4}{c|}{i-BAU \cite{zeng2022adversarial}}        & \multicolumn{4}{c}{SAU (\textbf{Ours})} \\
\midrule
Attack  & \multicolumn{1}{c}{ACC} & \multicolumn{1}{c}{ASR} & \multicolumn{1}{c}{R-ACC} & \multicolumn{1}{c|}{DER}  &  \multicolumn{1}{c}{ACC} & \multicolumn{1}{c}{ASR} & \multicolumn{1}{c}{R-ACC} & \multicolumn{1}{c|}{DER}  & \multicolumn{1}{c}{ACC}         & \multicolumn{1}{c}{ASR}  & \multicolumn{1}{c}{R-ACC}& \multicolumn{1}{c|}{DER}  & \multicolumn{1}{c}{ACC}  & \multicolumn{1}{c}{ASR} & \multicolumn{1}{c}{R-ACC}& \multicolumn{1}{c}{DER}  \\
\midrule
BadNets \cite{gu2019badnets} & $\textbf{97.99}$& $7.77$& $91.28$& $75.09$& $96.06$& $2.13$& $94.01$& $77.29$& $8.32$& $\underline{0.00}$& $8.51$& $34.48$& $95.02$& $0.00$& $\underline{94.53}$& $77.83$\\
Blended \cite{chen2017targeted} & $\textbf{98.82}$& $99.91$& $0.07$& $50.00$& $98.21$& $99.95$& $0.02$& $49.68$& $91.41$& $27.05$& $25.07$& $82.72$& $92.21$& $\underline{4.97}$& $\underline{38.73}$& $\underline{94.16}$\\
Input-Aware \cite{nguyen2020input} & $98.43$& $75.01$& $24.76$& $\underline{59.08}$& $nan$& $nan$& $nan$& $50.0$& $\underline{nan}$& $\underline{nan}$& $\underline{nan}$& $50.00$& $nan$& $nan$& $nan$& $50.00$\\
LF \cite{zeng2021rethinking} & $\underline{97.78}$& $98.52$& $1.19$& $50.05$& $97.72$& $98.67$& $1.11$& $50.0$& $88.25$& $0.99$& $\underline{22.55}$& $94.19$& $96.56$& $\underline{0.27}$& $8.03$& $\underline{98.71}$\\
SSBA \cite{li2021invisible} & $\underline{97.97}$& $99.03$& $0.82$& $50.08$& $97.36$& $91.17$& $7.14$& $53.71$& $13.48$& $\textbf{0.00}$& $12.57$& $57.36$& $91.96$& $0.37$& $\underline{66.48}$& $\underline{96.41}$\\
WaNet \cite{nguyen2021wanet} & $\textbf{98.63}$& $1.18$& $97.02$& $95.84$& $97.32$& $\underline{0.02}$& $94.08$& $96.36$& $98.04$& $0.02$& $97.63$& $\underline{96.41}$& $\underline{98.25}$& $0.07$& $\textbf{97.86}$& $96.39$\\
Average & $\textbf{98.27}$& $63.57$& $35.86$& $61.45$& $97.33$& $58.39$& $39.27$& $61.01$& $59.90$& $\underline{5.61}$& $33.27$& $66.45$& $94.80$& $\textbf{1.14}$& $\textbf{61.13}$& $\textbf{80.50}$\\

\bottomrule
\end{tabular}}
\end{table}


==> tables/gtsrb_vgg19_0_05.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h]
\centering
\caption{\textbf{GTSRB}, VGG19, 5.0\%}
\label{gtsrb_vgg19_05}
%%% Caption here
\setlength{\tabcolsep}{3pt} % Default value: 6pt
% \renewcommand{\arraystretch}{1.5} % Default value: 1
\scalebox{0.72}{
% \resizebox{\linewidth}{!}{
\begin{tabular}{c|cccc|cccc|cccc}
\toprule
Defense & \multicolumn{4}{c|}{No Defense}       & \multicolumn{4}{c|}{FP \cite{liu2018fine}}& \multicolumn{4}{c}{NC \cite{wang2019neural}}   \\ \midrule
Attack  & \multicolumn{1}{c}{ACC} & \multicolumn{1}{c}{ASR} & \multicolumn{1}{c}{R-ACC} & \multicolumn{1}{c|}{DER} & \multicolumn{1}{c}{ACC}         & \multicolumn{1}{c}{ASR}  & \multicolumn{1}{c}{R-ACC}& \multicolumn{1}{c|}{DER}  & \multicolumn{1}{c}{ACC}  & \multicolumn{1}{c}{ASR} & \multicolumn{1}{c}{R-ACC}& \multicolumn{1}{c}{DER}  \\
\midrule
BadNets \cite{gu2019badnets} & $96.04$& $55.7$& $6.25$&  N/A & $\underline{95.57}$& $91.89$& $6.84$& $49.77$& $48.28$& $\textbf{0.00}$& $\textbf{49.08}$& $53.97$\\
Blended \cite{chen2017targeted} & $96.35$& $99.13$& $0.29$&  N/A & $\textbf{96.15}$& $98.42$& $0.71$& $50.26$& $92.71$& $\underline{0.15}$& $\textbf{58.30}$& $\underline{97.67}$\\
Input-Aware \cite{nguyen2020input} & $96.98$& $41.38$& $57.51$&  N/A & $\textbf{97.80}$& $4.45$& $\underline{91.19}$& $68.46$& $97.06$& $\underline{0.06}$& $\textbf{95.68}$& $\underline{70.66}$\\
LF \cite{zeng2021rethinking} & $96.46$& $97.26$& $2.03$&  N/A & $\textbf{96.42}$& $96.79$& $2.40$& $50.22$& $94.83$& $2.85$& $\textbf{73.40}$& $96.39$\\
SSBA \cite{li2021invisible} & $96.1$& $98.2$& $1.08$&  N/A & $\textbf{95.95}$& $95.99$& $1.99$& $51.03$& $33.17$& $\textbf{0.00}$& $\underline{31.50}$& $67.63$\\
WaNet \cite{nguyen2021wanet} & $94.83$& $95.29$& $4.01$&  N/A & $\underline{97.36}$& $74.07$& $21.55$& $60.61$& $96.52$& $\underline{0.03}$& $\textbf{96.21}$& $\underline{97.63}$\\
Average & $96.13$& $81.16$& $11.86$&  N/A & $\textbf{96.54}$& $76.94$& $20.78$& $54.34$& $77.1$& $\textbf{0.52}$& $\textbf{67.36}$& $76.28$\\

\toprule

\toprule
Defense & \multicolumn{4}{c|}{NAD \cite{li2021neural}}  &  \multicolumn{4}{c|}{i-BAU \cite{zeng2022adversarial}}        & \multicolumn{4}{c}{SAU (\textbf{Ours})} \\
\midrule
Attack  & \multicolumn{1}{c}{ACC} & \multicolumn{1}{c}{ASR} & \multicolumn{1}{c}{R-ACC} & \multicolumn{1}{c|}{DER} & \multicolumn{1}{c}{ACC}         & \multicolumn{1}{c}{ASR}  & \multicolumn{1}{c}{R-ACC}& \multicolumn{1}{c|}{DER}  & \multicolumn{1}{c}{ACC}  & \multicolumn{1}{c}{ASR} & \multicolumn{1}{c}{R-ACC}& \multicolumn{1}{c}{DER}  \\
\midrule
BadNets \cite{gu2019badnets} & $\textbf{95.64}$& $59.63$& $18.62$& $49.8$& $94.28$& $\underline{1.11}$& $31.11$& $\textbf{76.42}$& $95.06$& $2.34$& $\underline{32.35}$& $\underline{76.19}$\\
Blended \cite{chen2017targeted} & $\underline{95.93}$& $93.79$& $3.36$& $52.46$& $93.42$& $\textbf{0.00}$& $\underline{29.55}$& $\textbf{98.10}$& $95.17$& $2.63$& $10.28$& $97.66$\\
Input-Aware \cite{nguyen2020input} & $\underline{97.70}$& $24.61$& $74.12$& $58.39$& $97.35$& $0.33$& $88.22$& $70.52$& $97.09$& $\textbf{0.00}$& $7.46$& $\textbf{70.69}$\\
LF \cite{zeng2021rethinking} & $\underline{96.41}$& $96.44$& $2.74$& $50.39$& $94.69$& $\textbf{0.06}$& $\underline{27.13}$& $\textbf{97.71}$& $94.85$& $\underline{0.33}$& $11.60$& $\underline{97.66}$\\
SSBA \cite{li2021invisible} & $\underline{95.65}$& $90.84$& $4.84$& $53.45$& $95.52$& $\underline{2.27}$& $\textbf{35.31}$& $\textbf{97.67}$& $95.01$& $7.41$& $19.80$& $\underline{94.85}$\\
WaNet \cite{nguyen2021wanet} & $\textbf{97.72}$& $8.66$& $\underline{88.89}$& $93.31$& $96.99$& $\textbf{0.00}$& $87.78$& $\textbf{97.65}$& $93.1$& $0.43$& $87.79$& $96.56$\\
Average & $\underline{96.51}$& $62.33$& $32.10$& $58.26$& $95.37$& $\underline{0.63}$& $\underline{49.85}$& $\textbf{84.01}$& $95.05$& $2.19$& $28.21$& $\underline{83.37}$\\

\bottomrule
\end{tabular}}
\end{table}

